DCdetector: Dual Attention Contrastive Representation Learning for Time Series Anomaly Detection

Time series anomaly detection is critical for a wide range of applications. It aims to identify deviant samples from the normal sample distribution in time series. The most fundamental challenge for this task is to learn a representation map that enables effective discrimination of anomalies. Reconstruction-based methods still dominate, but the representation learning with anomalies might hurt the performance with its large abnormal loss. On the other hand, contrastive learning aims to find a representation that can clearly distinguish any instance from the others, which can bring a more natural and promising representation for time series anomaly detection. In this paper, we propose DCdetector, a multi-scale dual attention contrastive representation learning model. DCdetector utilizes a novel dual attention asymmetric design to create the permutated environment and pure contrastive loss to guide the learning process, thus learning a permutation invariant representation with superior discrimination abilities. Extensive experiments show that DCdetector achieves state-of-the-art results on multiple time series anomaly detection benchmark datasets. Code is publicly available at https://github.com/DAMO-DI-ML/KDD2023-DCdetector.

==> Figures/case_study.tex <==
\begin{figure*}[htbp]
\centering
\includegraphics[width=0.97\textwidth]{img/casestudy/case_study.pdf}
 \vspace{-5mm}
\caption{Visualization of ground-truth anomalies and anomaly scores from DCdetector for different types of anomalies.} 
\label{fig:case} \vspace{-2mm}
\end{figure*}

==> tables/tab_SMD_Step1.tex <==
\begin{table*}[h!]
\begin{tabular}{c|llllllllll}
\hline \hline
\textbf{Dataset} & \multicolumn{10}{c}{\textbf{SMD (Step=1)}}                                                                                                                                                                                                                                    \\ \hline
\textbf{Metric}  & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Aff-P} & \multicolumn{1}{c}{Aff-R} & \multicolumn{1}{c}{R\_A\_R} & \multicolumn{1}{c}{R\_A\_P} & \multicolumn{1}{c}{V\_ROC} & \multicolumn{1}{c}{V\_PR} \\ \hline
AnomalyTrans     & 99.03                   & 87.28                 & 90.52                 & 88.87                  & 56.73                     & 90.88                     & 74.59                       & 70.44                       & 74.33                      & 70.20                     \\
DCdetector             & 98.92                   & 87.09                 & 87.57                 & 87.33                  & 52.11                     & 90.26                     & 71.29                       & 67.16                       & 69.78                      & 65.71                     \\ \hline \hline
\end{tabular}
\label{Tab: SMD Step1 results}
\caption{SMD Dataset Step=1 Results.}
\end{table*}
